Learning Barrier Functions with Memory for Robust Safe Navigation

Control barrier functions are widely used to enforce safety properties in robot motion planning and control. However, the problem of constructing barrier functions online and synthesizing safe controllers that can deal with the associated uncertainty has received little attention. This paper investigates safe navigation in unknown environments, using onboard range sensing to construct control barrier functions online. To represent different objects in the environment, we use the distance measurements to train neural network approximations of the signed distance functions incrementally with replay memory. This allows us to formulate a novel robust control barrier safety constraint which takes into account the error in the estimated distance fields and its gradient. Our formulation leads to a second-order cone program, enabling safe and stable control synthesis in a priori unknown environments.

==> tex/3_RRT-QP.tex <==
\section{Introduction of RRT-CBF Algorithm}

The RRT-CBF algorithm is first proposed by \cite{yang2019sampling}. The mean idea behind this algorithm is, instead of using explicit collision check and find nearest neighbors, a control barrier function(CBF) constraints based Quadratic Program(QP) is solved to generate a sequence of safe controls which can help find a collision-free trajectories. 

\subsection{Notations}

We first define the configuration space as $\mathcal{C}$, the obstacle set $\mathcal{C}_{obs} \subset \mathcal{C}$ and the goal set $\mathcal{C}_{goal} \subset \mathcal{C}$. A graph denoted as $\mathcal{G} = (\mathcal{V},\mathcal{E})$ where the set of vertices $\mathcal{V} \subset \mathcal{C}$ and the corresponding edges are $\mathcal{E}$. Each vertex in the graph is associated to a robot state $\boldsymbol{x} \in \mathbb{R}^n$, i.e. $\boldsymbol{x} \in \mathcal{C}$. We also need to define a set of admissible controls $\mathcal{U}$ where the control inputs draw from.

\subsection{Brief Introduction of RRT}
The original RRT algorithm can be stated as follows
\begin{itemize}
\item Sample a random point $\boldsymbol{x}_{rand}$ from the configuration space $\mathcal{C}$ using SAMPLEFREE function.
\item Find the nearest neighbor $\boldsymbol{x}_{nearest}$ in the graph $\mathcal{G}$ using NEAREST function.
\item Use the STEER function to move a distance $\epsilon$ from $\boldsymbol{x}_{nearest}$ towards $\boldsymbol{x}_{rand}$.
\item Denote the new point as $\boldsymbol{x}_{new}$ and run the COLLISIONFREE function to check if the new point hits an obstacle, if not, add $\boldsymbol{x}_{new}$ and the corresponding edge to the graph.
\item Terminate the algorithm once the goal is reached.
\end{itemize}

For each position $(x,y)$, we need to check whether it is in the goal region to end the algorithm. Here, we perform a goal region check by defining a GOALCHECK function which takes the current position $(x,y)$ and the goal position $(x_{goal},y_{goal})$ as inputs, and returns True if the euclidean distance between these two position is less than a pre-defined constant $\gamma$ and False otherwise. See Fig.~\ref{fig:RRT} for an illustration of the original RRT algorithm.

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\linewidth]{fig/RRT.png}
\caption{Original RRT Algorithm}
\label{fig:RRT}
\end{figure}

\subsection{Sampling Method in RRT-CBF Algorithm}
Instead of running the process above, two sampling processes will be performed in the RRT-CBF algorithm. First, we need to sample from the existing vertices in the graph i.e. $\boldsymbol{x}_e \in \mathcal{G}$ with a desired probability distribution $p_v$. In this study, given a graph $\mathcal{G}$ contains a set of vertices $\mathcal{V}$, we perform vertex sampling based on a uniform distribution i.e. we pick randomly in the existing vertices to determine how to expand the tree.

Second, some state variables that have less priority can be sampled to increase the probability of generating a collision-free trajectory. For example, the robot orientation of a unicycle model can be sampled for generating controls to steer the robot to the goal region. In this case, the vertices in the tree are only the information of the robot position. Therefore, in this study, we can perform state sampling on the orientation $\theta$ of the robot based on a Gaussian distribution 
\begin{equation}
\label{eq:guassian}
    p_s(\theta) = \frac{1}{\sqrt{2\pi\sigma^2}}e^{\frac{(\theta - \mu_{\theta})^2}{2\sigma^2}}
\end{equation}
where $\sigma^2$ is the variance and $\mu_{\theta}$ is the mean value of $\theta$. Since the state of the robot is given as $(x,y,\theta)$, and the goal position is denoted as $(x_{goal}, y_{goal})$ we can calculate the mean value of $\theta$ by
\begin{equation}
\label{eq:mean}
    \mu_{\theta} = \arctan(\frac{y_{goal}-y}{x_{goal}-x})
\end{equation}

\subsection{Control Techniques in RRT-CBF Algorithm}

In the obstacle avoidance problem, our goal is to calculate the control inputs $\boldsymbol{u} \in \mathcal{U}$ such that the robot can move on the collision-free trajectory. This safety constraint can be translated in terms of of the set of collision-free control inputs \cite{ames2016control}:
\begin{equation}\nonumber
\begin{aligned}
\mathcal{K}_{h}(x) &= \{\boldsymbol{u}\in U : L_f h(x) + L_g h(x)\boldsymbol{u} + \alpha h(x) \geq 0\} 
\end{aligned}
\end{equation}
in which $h$ is the barrier function. Selecting an input $\boldsymbol{u}$ in the above set will guarantee that the set $\mathcal{C} = \{x\in \mathbb{R}^m : h(x) \geq 0\}$ is invariant.

The barrier function for obstacle avoidance can be defined as follows \cite{glotfelter2017nonsmooth}
\begin{equation}
\label{eq:barrier}
    h^i(\boldsymbol{x}) = (x-x_o^i)^2 + (y-y_o^i)^2 - \delta^2 
\end{equation}
where $(x_o,y_o)$, $\delta$ represent the position of obstacles and the pre-defined safe distance respectively. The index i means we can handle multiple obstacles when needed.

The problem of calculating a control input $u$ belonging to the set $\mathcal{K}_h$ leads to a quadratic programming problem as follows
\begin{equation}
\label{eq:QP_rrt}
\begin{aligned}
\boldsymbol{u}^*(\boldsymbol{x}) &= \arg\min_{\boldsymbol{u}}  ||\boldsymbol{u}-\boldsymbol{u}_r||^2 \\
\text{s.t.} \, \, 
& L_f h_i(\boldsymbol{x}) + L_g h_i(\boldsymbol{x}) \boldsymbol{u} + \alpha h_i(\boldsymbol{x}) \geq 0 \\
& \boldsymbol{u}_{min} \leq \boldsymbol{u} \leq \boldsymbol{u}_{max}
\end{aligned}
\end{equation}
in which $\boldsymbol{u}_r$ is the reference control input and the $\alpha$ is a positive constant. The solution to this optimization problem is always in $\mathcal{K}_h$. Note that by considering a distance ahead the wheel axis in the robot model, the relative degree of the output $h(\boldsymbol{x})$ is one, and the corresponding Lie derivative has order one.

\subsection{RRT-CBF Algorithm}

To start the algorithm, we need to define the initial state of the robot $\boldsymbol{x}_0 \in \mathcal{C}$, the obstacle position $\boldsymbol{x}_{obs} \in \mathcal{C}_{obs}$ and the goal position $\boldsymbol{x}_{goal} \in \mathcal{C}_{goal}$. 

By running the goal region check we can see if the robot has reached the goal region, if not, perform vertex sampling from the existing graph $\mathcal{G}$. Then perform state sampling i.e. sampling the orientation $\theta$ of the robot using the information of current position and goal position. Once the above information is collected, a QP is solved to generate a sequence of controls which can generate a collision free trajectory to a new state $\boldsymbol{x}_{new}$ after a fixed time step $\Delta t$. The new point $\boldsymbol{x}_{new}$ can be added to the graph $\mathcal{G}$, and we repeat the above steps until the robot reaches the goal region.

Note that we also need to define a control reference $\boldsymbol{u}_r$ in the QP solver such that the robot can move directly to the goal when there are no obstacles in the environment. The control barrier function acts as a tool to steer the robot when the robot is about to hit the obstacles.


\begin{algorithm}[ht]
\SetAlgoLined
Define obstacle position: $\boldsymbol{x}_{obs} \in \mathcal{C}_{obs}$\;

Define start node: $\boldsymbol{x}_s \in \mathcal{C}$\;

Initialize the graph $\mathcal{G}$: $\mathcal{V} \leftarrow{\{\boldsymbol{x}_s\}}$; $\mathcal{E} \leftarrow{\emptyset}$;\

Define goal position: $\boldsymbol{x}_{goal} \in \mathcal{C}_{goal}$\;

 \While{not GOALCHECK($\boldsymbol{x}_{goal}$, $\boldsymbol{x}$)}{
  $\boldsymbol{x}_{state}$ $\leftarrow{SampleVertex(\mathcal{G},p_v)}$\;
  $\theta_{sample} \leftarrow{SampleState(\boldsymbol{x}_{state},\theta_{goal})}$\;
  $\boldsymbol{u}^* \leftarrow{SolveQP(\boldsymbol{x}_{state},\theta_{sample},\boldsymbol{u}_{ref},\boldsymbol{x}_{obs})}$\;
  \uIf{QP is feasible}{
  $path,\boldsymbol{x}_{new} \leftarrow{DriveRobot(\boldsymbol{u}^*,\boldsymbol{x}_{state},\Delta t)}$\;
   $\mathcal{V} \leftarrow{\mathcal{V} \cup \{\boldsymbol{x}_{new}\}}$; $\mathcal{E} \leftarrow{\mathcal{E} \cup path}$;}
\Return{ $\mathcal{G} = (\mathcal{V},\mathcal{E})$}
}
\caption{RRT-CBF}
\end{algorithm}
